Scale Mixtures of Neural Network Gaussian Processes

Recent works have revealed that infinitely-wide feed-forward or recurrent neural networks of any architecture correspond to Gaussian processes referred to as Neural Network Gaussian Processes (NNGPs). While these works have extended the class of neural networks converging to Gaussian processes significantly, however, there has been little focus on broadening the class of stochastic processes that such neural networks converge to. In this work, inspired by the scale mixture of Gaussian random variables, we propose the scale mixture of NNGPs for which we introduce a prior distribution on the scale of the last-layer parameters. We show that simply introducing a scale prior on the last-layer parameters can turn infinitely-wide neural networks of any architecture into a richer class of stochastic processes. With certain scale priors, we obtain heavy-tailed stochastic processes, and in the case of inverse gamma priors, we recover Student's $t$ processes. We further analyze the distributions of the neural networks initialized with our prior setting and trained with gradient descents and obtain similar results as for NNGPs. We present a practical posterior-inference algorithm for the scale mixture of NNGPs and empirically demonstrate its usefulness on regression and classification tasks. In particular, we show that in both tasks, the heavy-tailed stochastic processes obtained from our framework are robust to out-of-distribution data.

==> main/broadimpact.tex <==
% \section*{Broader Impact}
% \label{sec:broaderimpact}
% Our work is theoretical in nature, and has a limited short-term impact on the society. Its main beneficiaries would be machine-learning researchers. Our work may help them to deepen their understanding about deep neural networks and develop better probabilistic models that bring the benefits of deep learning and Gaussian processes together. 

==> main/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See section~}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See~\cref{sec:introduction}}
  \item Did you describe the limitations of your work?
    \answerYes{See~\cref{sec:conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Our work is theoretical in nature, and has a limited short-term impact on the society. Its main beneficiaries would be machine-learning researchers.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See~\cref{sec:preliminaries,sec:results}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See~\cref{sec:proofs}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See~\cref{sec:additional_experiments}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See~\cref{sec:additional_experiments}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See~\cref{sec:additional_experiments}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See~\cref{sec:additional_experiments}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See~\cref{sec:additional_information}}
  \item Did you mention the license of the assets?
    \answerYes{See~\cref{sec:additional_information}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See~\cref{sec:additional_information}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See~\cref{sec:additional_information}}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See~\cref{sec:additional_information}}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> main/figure.tex <==
\section{Figures}
\label{sec:figures}
Figure which shows correspondence with sampled data and exact prior.\\
\begin{figure}[t]
  \centering
  \includegraphics[width = 0.4\linewidth]{figures/exactprior.png}
  \caption{Correspondence with sampled initial output distribution and exact student t distribution.}
  \label{fig:exactprior.png}
\end{figure}\\
Figure which shows posterior mean and variance by using toy examples.
\begin{figure}[t]
  \centering
  \includegraphics[width = 0.4\linewidth]{figures/exactposterior.png}
  \caption{Exact posterior distributions of toy examples.}
  \label{fig:exactposterior.png}
\end{figure}
Figure which shows the distribution of the output of last layer trained model.
\begin{figure}[t]
    \centering
    \includegraphics[width = 0.6\linewidth]{figures/exactcorrespond_2.png}
    \caption{Distribution of the output of last layer trained model.}
    \label{fig:exactcorrespond1.png}
\end{figure}

Figure which shows the distribution of the output of whole layer trained model.
\begin{figure}[t]
    \centering
    \includegraphics[width = 0.6\linewidth]{figures/heavytailfeature.png}
    \caption{Distribution of the output of whole layer trained model.}
    \label{fig:exactcorrespond2.png}
\end{figure}

Figure which shows the distribution of few samples.
\begin{figure}[t]
    \centering
    \includegraphics[width = 0.6\linewidth]{figures/100alpha1-001beta4.png}
    \caption{Distribution of the output of few samples.}
    \label{fig:exactcorrespond3.png}
\end{figure}

Figure which shows the distribution of few samples.
\begin{figure}[t]
    \centering
    \includegraphics[width = 0.6\linewidth]{figures/correspond-1.pdf}
    \caption{Distribution of the output of few samples.}
    \label{fig:correspond-1.pdf}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width = 0.6\linewidth]{figures/sinx.pdf}
    \caption{\lyh{just for postioning2}}
    \label{fig:correspond-1.pdf}
\end{figure}

==> main/one_line_main_idea.tex <==
\section{One line main idea}
\label{sec:one line main idea}

Heavy tail process by giving a prior distribution to the variance of the initial normal distribution of the last layer nodes in the infinite width neural network.
